Hardness of Online Sleeping Combinatorial Optimization Problems

We show that several online combinatorial optimization problems that admit efficient no-regret algorithms become computationally hard in the sleeping setting where a subset of actions becomes unavailable in each round. Specifically, we show that the sleeping versions of these problems are at least as hard as PAC learning DNF expressions, a long standing open problem. We show hardness for the sleeping versions of Online Shortest Paths, Online Minimum Spanning Tree, Online $k$-Subsets, Online $k$-Truncated Permutations, Online Minimum Cut, and Online Bipartite Matching. The hardness result for the sleeping version of the Online Shortest Paths problem resolves an open problem presented at COLT 2015 (Koolen et al., 2015).

==> regret-reductions.tex <==
%!TEX root=shortest-path.tex
\section{Reducing Per-Action Regret to Ranking Regret}
\label{section:regret-reductions}

In this section we show that if the online combinatorial optimization problem of interest exhibits some special structure, then the per-action regret can be bounded by the ranking regret (and thus, by the policy regret as well). For this section, we assume that all element losses are in the range $[0, 1]$ rather than $[-1, 1]$; this assumption is only made for convenience and is easy to remove.


\begin{definition} \label{def:extensible}
An Online Combinatorial Optimization problem is said to have {\bf extensible structure}, if given any instance $(U, \D)$ of the problem and any integer $p > 0$, it is possible to construct, in $\poly(d, p)$ time, another instance $(U', \D')$ and an efficiently constructible map $\pi: \D' \rightarrow \D$ such that $U \subseteq U'$ and there are $2p$ distinguished elements of $U' \setminus U$ denoted by the labels in
\[ L = \bigcup_{i=1}^p \{(i, 0), (i, 1)\}\]
such that the decision set $\D'$ satisfies the following properties:
\begin{enumerate}
	\item For any $V' \in \D'$, we have $\pi(V') \subseteq V' \cap U$.

	\item For all $(b_1, b_2, \ldots, b_p) \in \{0, 1\}^p$ and any $V \in \D$, the action $\{(1, b_1), (2, b_2), \ldots, (p, b_p)\} \cup V$ is in $\D'$.
\end{enumerate}
It suffices for the map $\pi$ to be defined only for $V' \in \D'$ such that  $V' \subseteq U \cup L$ and $|V' \cap L| \leq p$.
\end{definition}

In most cases, $U'$ will simply be equal to $U \cup L$, and the map $\pi$ will simply be $\pi(V') = V' \cap U$, in which case the required conditions on the map $\pi$ are obviously met. We need the extra flexibility in the definition above to accommodate some problems such as Online $k$-Subsets and Online $k$-Truncated Permutations.

\begin{algorithm}[t]
\caption{\textsc{Algorithm $\algaction$ for minimizing per-action regret}
\label{algorithm:per-action-to-ranking}}
\begin{algorithmic}[1]
\REQUIRE An algorithm $\algrank$ for the online sleeping combinatorial optimization problem minimizing ranking regret, and an instance $(U, \D)$ of the problem.
\STATE Construct the instance $(U', \D')$ with $p := \lceil \log_2(T) \rceil$ from Definition~\ref{def:extensible} and the map $\pi: \D' \rightarrow \D$, and run algorithm $\algrank$ on it.
\FOR{$t=1,2,\dots,T$}
\STATE Receive the set of sleeping elements $S_t \subseteq U$.
\STATE Let $(b_1, b_2, \ldots, b_p) \in \{0, 1\}^p$ be the encoding of $t$ in binary.
\STATE Set the sleeping elements for $\algrank$ to be $S_t' = S_t \cup \{(i, 1-b_i)\ |\ 1 \leq i \leq p\} \cup (U' \setminus (U \cup L))$.
\STATE Obtain an awake action (if one exists) $V_t' \in \D'$ by running $\algrank$; if there are no awake actions, skip this round.
\STATE Play the action $V_t = \pi(V_t')$, and receive losses $\ell_t(e)$ of all awake elements $e \in U \setminus S_t$.
\STATE In algorithm $\algrank$, set the loss of all awake elements the awake elements $e \in U' \setminus S_t'$ as follows:
	\[
	\ell_t'(e) = \begin{cases}
		\ell_t(e) & \text{ if } e \in U \\
		0 & \text{ if } e \in L
	\end{cases}
	\]
\ENDFOR
\end{algorithmic}
\end{algorithm}



\begin{theorem} \label{thm:regret-reduction}
	Suppose there is an algorithm $\algrank$ for an online sleeping combinatorial optimization problem with extensible structure with ranking regret bounded by $\poly(d) T^{1-\delta}$, for some constant $\delta \in (0, 1)$. Then there is an algorithm $\algaction$ for the problem with per-action regret bounded by $\poly(d, \log(T)) T^{1-\delta}$.
\end{theorem}
\begin{proof}
	$\algaction$ is given in Algorithm~\ref{algorithm:per-action-to-ranking}. First, we note that in any round $t$, if there is any awake action $V \in \D$ for the base instance $(U, \D)$, then the action $\{(i, b_i)\ |\ 1 \leq i \leq p\} \cup V$ is awake for the derived instance $(U', \D')$, where $(b_1, b_2, \ldots, b_p) \in \{0, 1\}^p$ is the binary encoding of $t$. Thus, in step 6 of algorithm $\algaction$, if there are no awake actions for the derived instance, then there are certainly no awake actions for the base instance, and so it is valid to skip the round.

	Next, note that in every round $t$, we have
	\[ \ell_t(V_t)\ =\ \ell_t(\pi(V_t'))\ \leq\ \ell_t(V_t' \cap U)\ =\ \ell_t'(V_t' \cap U)\ \leq\ \ell_t'(V_t'),\]
	because all elements have non-negative losses, and since $\pi(V_t') \subseteq V_t' \cap U$.

	Now, let $V \in \D$ be an arbitrary action with respect to which we want to measure per-action regret of algorithm $\algaction$. Consider the following ranking of actions in $\D'$. For every round $t$, define
	\[
		V_t^\star = \begin{cases}
		V & \text{ if } V \in \A_t \\
		\arg\min_{X \in \A_t} \ell_t(X) & \text{ otherwise,}
	\end{cases}
	\]
	and define the ranking where for $t = 1, 2, \ldots, T$, if $(b_1, b_2, \ldots, b_p) \in \{0, 1\}^p$ is the encoding of $t$ in binary, the $t$-th ranked action is
	\begin{equation} \label{eq:ranking}
		\{(1, b_1), (2, b_2), \ldots, (p, b_p)\} \cup V_t^\star
	\end{equation}
	After these top $T$ actions, the remaining actions in $\D'$ are ranked arbitrarily.

	It is easy to check that in each round $t$, the top ranked awake action is exactly the one given in (\ref{eq:ranking}). Since elements in $L$ always have $0$ loss, we conclude from the definition of $V_t^\star$ that in each round $t$, the loss of this ranking equals the loss of $V$ when $V$ is awake, and is at most the loss of $V_t$ when $V$ is not available. Thus, the ranking regret of $\algrank$ with respect to this ranking is an upper bound on the per-action regret of $\algaction$ with respect to $V$. Since the size of $U'$ is bounded by $\poly(d, \log T)$, we conclude that the per-action regret of $\algaction$ is bounded by $\poly(d, \log(T)) T^{1-\delta}$.	
\end{proof}

\subsection{Stochastic I.I.D. Sleeping Patterns} 

In the above proof, the sleeping patterns for the elements in $L$ are generated in a pre-determined order (viz. the binary encodings of the rounds). It is easy to change the proof so that these sleeping patterns are generated in an i.i.d. fashion, based on the observation that the only use of the patterns in the proof is to guarantee a unique sleeping pattern in each round. So one can use $p = 2\lceil \log_2(T) \rceil$, and generate a uniformly random bit pattern $(b_1, b_2, \ldots, b_p) \in \{0, 1\}^p$ in each round and use it to determine the sleeping pattern instead. Since there are only $T$ rounds, the choice of $p$ implies that the chance that any sleeping pattern is repeated is at most $\frac{1}{T}$. Conditioned on there being no repeated sleeping pattern, the regret analysis of the proof goes through, and thus the expected per-action regret is still bounded by $\poly(d, \log(T)) T^{1-\delta}$.	

\subsection{Extensible Structure for Specific Problems}

Now we apply Theorem \ref{thm:regret-reduction} to prove that all the online
sleeping combinatorial optimization problems considered in this paper have extensible structure, which implies that an algorithm minimizing ranking (or policy regret) for any of these problems can be used to minimize per-action regret as well.

\subsubsection{Online Shortest Path Problem}

Given an input graph $G = (V, E)$ with source and sink nodes denoted $s$ and $t$ respectively, and a positive integer $p$, the new instance graph $G' = (V', E')$ is constructed as follows. We add $p$ new nodes $v_1, v_2, \ldots, v_p$, and add 2 parallel edges between nodes $v_i$ and $v_{i+1}$ labeled $(i, 0)$ and $(i, 1)$, for $i = 1, 2, \ldots, p-1$, and 2 parallel edges labelled $(p, 0)$ and $(p, 1)$ between nodes $v_p$ and $s$. We make $v_0$ the new source node, and $t$ remains the sink node. Thus the new ground set of edges is $E' = E \cup L$, and the map $\pi$ is defined to be $\pi(P') = P' \cap E$ for any path $P'$ connecting $v_0$ to the sink node $t$. It is easy to check that this construction satisfies the required properties.

\subsubsection{Online Minimum Spanning Tree Problem}

Given an input graph $G = (V, E)$ and a positive integer $p$, the new instance graph $G' = (V', E')$ is constructed as follows.  We add $p$ new nodes $v_1, v_2, \ldots, v_p$, and add 2 parallel edges between nodes $v_i$ and $v_{i+1}$ labeled $(i, 0)$ and $(i, 1)$, for $i = 1, 2, \ldots, p-1$, and 2 parallel edges labelled $(p, 0)$ and $(p, 1)$ between nodes $v_p$ and an arbitrary node $s \in V$. Thus the new ground set of edges is $E' = E \cup L$, and the map $\pi$ is set to $\pi(T') = T' \cap E$ for any spanning tree $T'$ in $G'$. It is easy to check that this construction satisfies the required properties.

\subsubsection{Online \texorpdfstring{$k$}{k}-Subsets Problem}

Given input parameters $k$ and $d$ for the Online $k$-Subsets Problem and a positive integer $p$, the new instance is constructed as follows. We add $2p$ new elements with labels in $L$, and set $k' = k + p$ and $d' = d + 2p$, and consider the Online $k'$-Subsets Problem on these $d'$ elements. To construct the map $\pi$, let $V'$ be any subset of size $k'$ of the new ground set $U'$, and define $\pi(V')$ to be any subset of size $k$ of $V' \cap U$: we have $|V' \cap U| \geq k$ since we may assume that $V'$ has at most $p$ elements from $L$. It is easy to check that this construction satisfies the required properties.

\subsubsection{Online \texorpdfstring{$k$}{k}-Truncated Permutations Problem}

Given input parameters $k$ and $m$ for the Online $k$-Truncated Permutations Problem and a positive integer $p$, the new instance is constructed as follows. We add $p$ new elements $u_1, u_2, \ldots, u_p$ to the left hand side of the bipartite graph, and $2p$ new elements $v_{i, 0}, v_{i, 1}$ for $i = 1, 2, \ldots, p$ on the right hand side. We label the edges connecting the node $u_i$ to the nodes $v_{i, 0}$ and $v_{i, 1}$ with $(i, 0)$ and $(i, 1)$ respectively. We then set $k' = k + p$ and $m' = m + 2p$ and consider the Online $k'$-Truncated Permutations Problem on this bipartite graph. To construct the map $\pi$, let $M'$ be any maximal matching in the new graph, and we may assume that $M'$ has no edges connecting any of the nodes on the left hand side of the original graph to the new nodes $v_{i, b}$ for $1 \leq i \leq p$ and $b \in \{0, 1\}$. Then we can define $\pi(M') = M' \cap E$ which is a maximal matching in the original graph. It is easy to check that this construction satisfies the required properties.

\subsubsection{Online Bipartite Matching}

Given an input bipartite graph $G = (V, E)$, the new instance graph $G' = (V', E')$ is constructed by simply adding $p$ new pairs of nodes labelled $u_i$ and $v_i$ with 2 parallel edges labelled $(i, 0)$ and $(i, 1)$ between them, for $i = 1, 2, \ldots, p$. Thus the new ground set of edges is $E' = E \cup L$, and the map $\pi$ is set to $\pi(M') = M' \cap E$ for any maximal matching $M'$ in $G'$. It is easy to check that this construction satisfies the required properties.

\subsubsection{Online Minimum Cut}

Given an input graph $G = (V, E)$ with designated vertices $s$ and $t$ that we have to separate via a cut and a positive integer $p$, the new instance graph $G' = (V', E')$ is constructed by simply adding $2p$ new parallel edges labelled $(i, 0)$ and $(i, 1)$ for $i = 1, 2, \ldots, p$ connecting $s$ to $t$, with the same designated vertices $s$ and $t$ needing to be separated. Thus the new ground set of edges is $E' = E \cup L$, and the map $\pi$ is set to $\pi(C') = C' \cap E$ for any cut $C'$ separating $s$ from $t$. It is easy to check that this construction satisfies the required properties.

